Searching for Compact Obscured Nuclei in Compton Thick AGN

Compact Obscured Nuclei (CONs) are heavily obscured infrared cores that have been found in local (ultra)luminous infrared galaxies (U/LIRGs). They show bright emission from vibrationally excited rotational transitions of HCN, known as HCN-vib, and are thought to harbor Compton Thick (CT, $N_{\text{H}} \geq 10^{24}$ cm$^{-2}$) active galactic nuclei (AGN) or extreme compact starbursts. We explore the potential evolutionary link between CONs and CT AGN by searching for CONs in hard X-ray-confirmed CT AGN from the Great Observatories All-sky LIRG Survey (GOALS). Here, we present new Atacama Large Millimeter/submillimeter Array Band 6 observations that targeted HCN-vib emission in four hard X-ray-confirmed CT AGN. We analyze these objects together with literature HCN-vib measurements of five additional hard X-ray-confirmed CT AGN from the GOALS sample. We do not detect any CONs in this combined sample of nine CT AGN. We then explore a proposed evolutionary sequence in which CONs evolve into X-ray-detectable CT AGN once outflows and feedback reduce the column densities of the enshrouding gas. We find, however, no evidence of well-developed dense molecular outflows in the observed CT AGN. While this could suggest that CT AGN are not universally linked to CONs, it could also be explained by a short duty cycle for molecular outflows.

==> source_prop.tex <==
% \begin{deluxetable}{ccc}[h!]
% % \tabletypesize{\large}
% \tablecaption{HCN-vib Upper Limits and Continuum Properties}
% \tablehead{ \colhead{Source} &  \colhead{$\Sigma_{\text{HCN-vib}}$} &  \colhead{$S_{\text{1mm}}/\Delta\Omega$}   \\ 
% \colhead{} &  \colhead{($L_\odot$ / pc$^2$)} & \colhead{(mJy/arcsec$^2$)} } 
% \startdata
% NGC 4922N  &  $<0.026$ & 10.6 $\pm$ 0.3\\
% NGC 7130  &  $<0.026$  & 113.3 $\pm$ 7.5 \\
% NGC 7674  &  $<0.035$ & 9.6 $\pm$ 0.3  \\
% NGC 6921 & $<0.028$  &  2.3 $\pm$ 0.3
% \enddata
% \end{deluxetable}
